EigenNetworks

Many applications donot have the benefit of the laws of physics to derive succinct descriptive models for observed data. In alternative, interdependencies among $N$ time series $\{ x_{nk}, k>0 \}_{n=1}^{N}$ are nowadays often captured by a graph or network $G$ that in practice may be very large. The network itself may change over time as well (i.e., as $G_k$). Tracking brute force the changes of time varying networks presents major challenges, including the associated computational problems. Further, a large set of networks may not lend itself to useful analysis. This paper approximates the time varying networks $\left\{G_k\right\}$ as weighted linear combinations of eigennetworks. The eigennetworks are fixed building blocks that are estimated by first learning the time series of graphs $G_k$ from the data $\{ x_{nk}, k>0 \}_{n=1}^{N}$, followed by a Principal Network Analysis procedure. The weights of the eigennetwork representation are eigenfeatures and the time varying networks $\left\{G_k\right\}$ describe a trajectory in eigennetwork space. These eigentrajectories should be smooth since the networks $G_k$ vary at a much slower rate than the data $x_{nk}$, except when structural network shifts occur reflecting potentially an abrupt change in the underlying application and sources of the data. Algorithms for learning the time series of graphs $\left\{G_k\right\}$, deriving the eigennetworks, eigenfeatures and eigentrajectories, and detecting changepoints are presented. Experiments on simulated data and with two real time series data (a voting record of the US senate and genetic expression data for the \textit{Drosophila Melanogaster} as it goes through its life cycle) demonstrate the performance of the learning and provide interesting interpretations of the eigennetworks.

==> simulatedexp.tex <==
%\subsection{Simulated Data}
 We explain how we generate the time varying networks $\left\{\A_k\right\}$ and the data $\left\{\x_k\right\}$, $k=1,\cdots, K$. For lack of space, we report results for the following choice of parameters: number of nodes $N=25$; number of eigennetworks $R=2$; number of change points $S=1$; order of the autoregressive $M=2$; time window $K=250$. From equation~\eqref{eq:autoreg}, $\A_k=\left(\A_{k,1}\, \A_{k,2}\right)$. At each~$k$, $\A_k$ will be a weighted linear combination of~$R=2$ eigennetworks. From equation~\eqref{eq:eigencomponents}, at each~$k$, we need the eigenfeature or weight $\c_{k}=\left(c_{k}^{(1)} \, c_{k}^{(2)}\right)^\top \in \Rbb^{2 \times 1}$ and the two eigennetworks $\B^{(r)} \in\Rbb^{2\times 25}$, $r=1,2$.
 
 We generate the $R=2$ eigennetworks $\B^{(r)}\in\Rbb^{25\times 50}$ as weighted Erd\"{o}s-R\'{e}nyi networks with probability of an edge $.025$ and asymetric random edge weights drawn from a normal distribution $\Ncal(0,1)$  with diagonal entries uniformly generated in $[1,2)$. In this study, we keep the eigennetworks fixed across the time window $k=1,\cdots,250$. We then generate changepoints  uniformly at random in $\left[\frac{K-M}{S+1}(i-\frac{1}{8}),\frac{K-M}{S+1}(i+\frac{1}{8})\right)$ for $i=1,\ldots,S$ where $S$ is the number of changepoints (in this study $S=1$). At each time step~$k$, the eigenfeatures or weights $\c_{k}=\left(c_{k}^{(1)} \, c_{k}^{(2)}\right)^\top$ of the linear combination are the sum of a fixed level and a sinusoidal term. Because we have two eigennetworks, we have two weights at each~$k$. The fixed level of each weight $c_{k}^{(j)}$, $j=1,2$, and in between changepoints, is kept constant and is drawn uniformly at random from $[2\,\,4)$. The parameters of each of the two sinusoids do not change in the whole time window, i.e., they remain the same across the changepoint. The amplitude of each sinusoid is drawn uniformly from the interval $[1/4\,\,1/2)$, the period being the same for both and equal to~$250$, the duration of the time window. The phase of one of the sinusoids is taken to be zero and that of the other to be $\pi/4$. By linear combination of the two (fixed)  Erd\"{o}s-R\'{e}nyi $\B^{(r)}$ eigennetworks weighted by the $K=250$ eigenfeatures $\c_{k}=\left(c_{k}^{(1)} \, c_{k}^{(2)}\right)^\top$ so generated, we created $K=250$ time varying networks $\A_k=\left(\A_{k,1}\, \A_{k,2}\right)$, each of size $N=25\times50=MN$. These time varying networks $\left\{\A_k\right\}$ are all created by the same structure (fixed eigennetowrks), but vary continuously because of the sinusoidal terms in the features $\c_{k}=\left(c_{k}^{(1)} \, c_{k}^{(2)}\right)^\top$, except at the changepoint when the weights jump as the magnitude levels and the amplitudes of the sinusoids jump. This makes it a fairly difficult setting conceptually, as the structure of the eigennetworks remains constant. We also generated data supported on these networks according to an autoregressive process of order $M=2$. 



\begin{figure}[thb]
	\includegraphics[width=0.95\columnwidth]{toy_true_vs_est.eps}
	\caption{Graphs of the top 25 edges of the estimated and true eigennetworks}
	\label{fig:pna:toy_true_vs_est}
\end{figure}
%
Figure~\ref{fig:pna:toy_true_vs_est} shows the true and estimated eigennetworks used to generate the data. Structure-wise, the eigennetworks are estimated fairly well; the first eigennetwork has a probability of false alarm\footnote{Probability of false alarm of an edge is the probability that an estimated edge is not present in the true eigennetwork. Likewise, probability of detection is the probability that an edge in the true eigennetwork is present in the estimated eigennetwork. Because edges are weighted, we threshold the weights,}  $P_{\scriptsize\textrm{FA}}=0.029$ and a probability of detection $P_{\scriptsize\textrm{D}}=0.73$, while the second has a $P_{\scriptsize\textrm{FA}}=0.036$ and $P_{\scriptsize\textrm{D}}=0.72$. For visualization, we desire low false alarm to avoid clutter and end up at an operating point with conservative detection. We also note that this is a difficult setting since both networks are strongly active in the first half of the time series while less active in the second half. Thus the two networks are difficult to distinguish in noise, and we see some edges present in both estimates that are only present in one true eigennetwork (e.g., between nodes 16 and 20). A fuller characterization of the ROC would be an interesting direction for future work.

\begin{figure}[thb]
	\includegraphics[width=0.95\columnwidth]{toy_graph_bigger.eps}
	\caption{Graphs of the top 50 edges}
	\label{fig:pna:toy_graphs}
\end{figure}
%
Figure~\ref{fig:pna:toy_graphs} shows that near the detected changepoint, using the same sparsity regularization parameter $\lambda$, the networks estimated with the changepoints are better able to capture the weights on either side of the changepoint, while the central estimator seems to average too strongly across the changepoint, resulting in weaker edges. We show in figure~\ref{fig:pna:toy_plots} the performance of our estimation method as compared to the central estimator for $\lambda=0.1$ and $w^{(c)}_{kj}\propto e^{-\frac{(j-k)^2}{200}}$.
\begin{figure}[thb]
	%\hspace{-0.075\columnwidth}
	\includegraphics[width=1.1\columnwidth]{tvgraph_vs_central2.eps}
	\caption{Time series of elements of graph adjacency matrix and corresponding errors}
	\label{fig:pna:toy_plots}		
\end{figure}
In figure~\ref{fig:pna:toy_plots} each line represents the time series of the weights corresponding to one edge. We see that using our method, the changepoint is estimated well, with the overall error comparing favorably to that of the normal central kernel estimate. We note that the estimated magnitudes of the edge weights for the graph are shrunken as a result of the regularization, and there is some bias towards $0$ at the boundaries. This suggests an extension of the method would be to let the regularization parameter $\lambda$ vary through the interval rather than stay constant. A proper time profile of the $\lambda$ value would be of interest.

